Physics-informed GANs for Coastal Flood Visualization

As climate change increases the intensity of natural disasters, society needs better tools for adaptation. Floods, for example, are the most frequent natural disaster, but during hurricanes the area is largely covered by clouds and emergency managers must rely on nonintuitive flood visualizations for mission planning. To assist these emergency managers, we have created a deep learning pipeline that generates visual satellite images of current and future coastal flooding. We advanced a state-of-the-art GAN called pix2pixHD, such that it produces imagery that is physically-consistent with the output of an expert-validated storm surge model (NOAA SLOSH). By evaluating the imagery relative to physics-based flood maps, we find that our proposed framework outperforms baseline models in both physical-consistency and photorealism. While this work focused on the visualization of coastal floods, we envision the creation of a global visualization of how climate change will shape our earth.

==> parking_lot.tex <==
ABSTRACT
%%%ToDo:  discussion to keep in mind in journal version or add summary to appendix:
% we resolved that the information from elevation maps is baked into the segmentation masks. I was suggesting we would want to include the topography values along with the segmentations as multiple “maps” (i.e. multiple constraint matrices), but I believe we didn’t get to those experiments
% Christian Requena  1 day ago
% I see there is two "elevation maps" that we might be mixing.
% I think the elevation map Natalia was talking about was refering to "water depth" to replace the binary segmentation mask. This is very hard to imposible, as we would need high-res water depth (either SAR or model output) for the exact time the satellite image was taken.
% Then there is adding terrain elevation as an extra constraining variable. This one is totally doable and something we could have tried. The only limiting factor was that it implies we know the flood models are not optimal and we would be intending to improve the flood extent predictions instead of just projecting their outputs as a photorealistic visualization.
% (edited)
% Alexander Lavin  1 day ago
% this figure from one of my papers (apologies for the shameless plug :wink:) illustrates the concept of multiple “maps”, in this case for a multiobjective path planning algorithm, where each map added more physical constraints to the solution space.

%\newcommand\myfigure{%
%  \vspace{-.3in}
%  \centering
%  \begin{subfigure}{.7\columnwidth}
%      \centering
%      \includegraphics [trim=0 .3 0 0, clip, width=1.\textwidth, angle = 0]{figures/results_overview}
%      \vspace{.02in}
      %\caption{Before training}
%  \end{subfigure}
%\caption[related works]{We generated physically-consistent satellite imagery of coastal flood events.}  
%\captionof{figure}{We generated the first physically-consistent satellite imagery of coastal flood events.}
%\label{fig:results_overview}
%}

%ToDo: make it work, should go before maketitle and after keyworkds in ACM template.  LaTeX Error: Environment teaserfigure undefined.
% \begin{teaserfigure}%[htbp!]%t]
% \begin{center}
%   \centering
%   \begin{subfigure}{.7\columnwidth}
%       \centering
%       \includegraphics [trim=0 0 0 0, clip, width=1.\textwidth, angle = 0]{figures/results_overview}
%       \vspace{.02in}
%       %\caption{Before training}
%   \end{subfigure}
% \caption[related works]{We generated physically-consistent satellite imagery of coastal flood events.} \label{fig:results_overview} 
% \end{center}
% \end{teaserfigure}

    %The proposed visualizations will enable a variety of stakeholders in climate resilience planning and disaster preparedness to communicate flood risks to decision-makers.
  %Floods rank as top most frequent and destructive disasters resulting in massive human and infrastructure losses. In an era of climate change, innovative approaches are needed to address various short- and long-term aspects of these disasters. In this regard, we utilize two Generative Adversarial Networks (GAN) based approaches, namely Pix2Pix and BicycleGAN to predict photo realistic imagery for coastal flood events. We also constrain our GAN models using SLOSH, a physics based flood extent model. Given that our predictions consist of both image quality and model accuracy considerations, we develop a novel metric, namely the FVIPS1 score, which is a harmonic sum of the LPIPS and IoU metrics. We used the xBD dataset and focused on recent US east coast storm events namely Hurricane Harvey, Matthew, Michael and Sandy. The created imagery achieves XX-on physical consistency, as measured by Intersection over Union (IoU) over the flood extent, and XX- on photorealism as measured by LPIPS. All code will be made publicly available at \url{https://gitlab.com/frontierdevelopmentlab/fdl-us-2020-earth-engine}.


INTRO 


%The proposed visualizations will enable a variety of stakeholders in climate resilience planning and disaster preparedness to communicate flood risks to decision-makers.

%To mitigate the impacts of these intensifying events, various technologies are being utilized ranging from physical models to in-situ measurements. Earth observations (EO) have recently emerged as an innovative means to monitor and map flood impacts in near-real time, though such observations are limited due to factors such as insufficient coverage, clouds and low-resolution, especially in the context of urban flood events. In the context of climate change change impacts such as floods, and towards addressing these gaps in the short- and long-term, we develop a machine learning/AI based approach to predict photo-realistic images of the future. Broadly speaking, our approach is aimed to not only aid disaster response in the context of climate change response, but also assist in climate resilience related areas such as urban planning and sustainable development.   

%As stakeholders ranging from local to national governments cope with increased flood risks due to climate change, visual explanations can aid their decision-making process []. And while today’s flood modeling capabilities include both informative, color-coded maps, as well as intuitive, street-level images, as displayed in\cref{fig:related_works}, decision-makers would benefit from imagery that is both informative and intuitive. Accordingly, the Frontier Development Lab’s Earth Intelligence Engine team produced satellite images of future coastal floods: physics-informed, photorealistic images that look like real satellite imagery. The generated visualizations, as shown in~\cref{fig:results_overview} enable a variety of stakeholders in climate resilience planning and disaster preparedness to communicate flood risks to decision-makers. 


%To mitigate the impacts of these intensifying events, various technologies are being utilized ranging from physical models to in-situ measurements. Earth observations (EO) have recently emerged as an innovative means to monitor and map flood impacts in near-real time, though such observations are limited due to factors such as insufficient coverage, clouds and low-resolution, especially in the context of urban flood events. In the context of climate change change impacts such as floods, and towards addressing these gaps in the short- and long-term, we develop a machine learning/AI based approach to predict photo-realistic images of the future. Broadly speaking, our approach is aimed to not only aid disaster response in the context of climate change response, but also assist in climate resilience related areas such as urban planning and sustainable development.   

RELATED WORKS

%, rather than trying to improve on their predictions via embedding physics (e.g., hydrological modeling) in the DNN %GAN architecture. 

%, and we focus on GANS, as they produce more photorealistic imagery in general. % Our proposed EIE pipeline consists of using additional information from physics models providing flood extent. 

%GAN to adversarially learn an image-to-image transformation~\cite{Chen_20}. Variational Autoencoders (VAE) \cite{kingma2013auto} are another class of generative vision models, with recent works using physical conditioning (e.g. GPPVAE) ~\cite{casale2018gaussian}. % A similar VAE-based approach that does not assume iid data is GPPVAE~\cite{casale2018gaussian}. 

%\section{Related work: Visualizations of future coastal floods}
%Existing visualizations of coastal floods are either informative, i.e., color-coded pixels on a map, or intuitive, i.e., photorealistic street-view imagery. The informative, color-coded map visualization, displayed in~\cref{fig:related_works}a) (SLOSH Hazard Map,~\cite{Jelesnianski_92}), can be overlayed with other geospatial layers (e.g., evacuation routes) conveys a quick overview of the flood extent. According to expert interviews, however, its color-coding of inundation height can complicate communication to non-technical stakeholders, delaying decision-making in time-critical scenarios. %(Radovan and de Suarez, 2020)\blXX{missing}. Street-view imagery,  displayed in~\cref{fig:related_works}b)~\cite{Schmidt_2019}, on the other hand, can intuitively convey local impact and evoke visceral emotions. However, it remains too local for street-level disaster planning and response. To the extent of the authors knowledge, the proposed physically-consistent visualization is the first to combine the two, enabling a variety of  stakeholders  in  climate  adaptation  planning  and disaster  preparedness  to  quickly  gauge the city-scale  impacts  of  coastal  floods.

%Generative adversarial networks (GANs)~\cite{Goodfellow_2014} are a kind of deep neural network (DNN) that achieved significant success in image generation \cite{brock2018large} and many other applications, including image prediction of photorealistic satellite images to represent the effects of climate change \cite{requena2019predicting}.

% moved to experiments %%%%%%%
%%%%%%%%%%%%%%%%%%%%%%

%\textbf{Physical consistency in the model architecture of GANs.} \blXX{combine with 2.2}

%Most generative models use a GAN to adversarially learn an image-to-image transformation~\cite{Chen_20}. Variational Autoencoders (VAE) \cite{kingma2013auto} are another class of generative vision models, with recent works using physical conditioning (e.g. GPPVAE) ~\cite{casale2018gaussian}. % A similar VAE-based approach that does not assume iid data is GPPVAE~\cite{casale2018gaussian}. 
%However, most of them mainly use RGB data as input. For instance, Pix2PixHD \cite{Wang18pix2pixHD} is a high-resolution generative model that allows for high-resolution image generation. However, its decoder only is able to produce a single deterministic output image for a given input. BicycleGAN \cite{Zhu17BicycleGAN} is another performant image to image translation method that as Pix2PixHD, allows to take advantage of paired image to image translation in a supervised manner. The advantage is that it is composed of a VAE module that allows to quantify uncertainty in the output model, since it does not allow to create 1-to-1 mapping for a given input but 1-to-many, truly learning the data distribution able to map among both domains.


%In this work we raise the challenge of generating physically-consistent imagery, here defined as satellite imagery that accurately depicts the flood extent as predicted by scientifically validated storm surge models. %, and we focus on GANS, as they produce more photorealistic imagery in general. % Our proposed EIE pipeline consists of using additional information from physics models providing flood extent. 

% \begin{itemize}
%     \item The  first  physically-consistent  visualization  of  coastal  flood  model  outputs  as  high-resolution, photorealistic satellite imagery.
%     \item Flood Visualization Plausibility Score (FVPS): A novel metric to evaluate the photorealism and validity of physically-modeled flood extent in generated imagery. 
%     \item A framework to generate physically-consistent visualizations of climate extremes
% \end{itemize}

MATERIALS AND METHODS
%As shown in Figure 4, we trained a generative vision model on image triplets, so the model learns to go from pre-flooding to post-flooding images based on flood extent inputs. After training, we generated future-flood images by replacing “ground truth” flood extents with a flood map, generated by a scientifically validated storm surge model.

%Our model generates post-flooding imagery given pre-flooding imagery and a flood extent map, as shown in \cref{fig:model_architecture}.

%Because xBD offers pre- and post-flooding image pairs, we focus on conditional generative models for paired image translation (e.g., Pix2Pix~\cite{Isola_2017}, instead of more demanding unpaired image translation models (e.g., CycleGAN~\cite{zhu2017unpaired}).
%\begin{itemize}
    %\item Photorealism: The ability to output images that are interpretable by and meaningful to humans, i.e. with high photorealism; and,
    %\item Sample Diversity: The ability to generate an ensemble of post-disaster imagery (ensemble forecasting with aleatoric and epistemic uncertainty management). 
%\end{itemize}
%One state-of-the art model, Pix2PixHD~\cite{Wang_2018}, achieves high photorealism, but the model’s output is deterministic, impeding the creation of an ensemble forecast. On the other hand, architectures such as BicycleGAN~\cite{Zhu17BicycleGAN} enforce the variational constraint on the bottleneck in order to avoid mode-collapse, allowing the model to create ensemble forecasts; however, we expect BicycleGAN to generate less photorealistic imagery. Still, as displayed in Fig. 3, we are close to achieving our safe goal of generating images without physics-based inputs. In particular, we have trained Pix2PixHD and BicycleGAN to generate post-flooding imagery in a Google Cloud instance. 

%When using generative vision models to generate physically-plausible, photorealistic, post-flooding images, architecture selection hinges on two criteria: photorealism and physical consistency.

%IoU measures the overlap of the input flood mask and a generated flood mask of the output imagery. There exists reliable model for flood classification from pure RGB imagery. Hence, a segmentation model (based on Pix2pix) has been trained on ${\sim}100$ hand-labelled images to do pixel-wise flood segmentation from RGB imagery and generated the output flood mask. 

%For instance, MMD and 1-NN evaluate the ability of the model to discriminate between real versus fake images, its sensitivity to mode dropping and collapse, and computational efficiency. 
%the 2.b.) IoU of flood segmentation and 1b) a learned perceptual loss (here, LPIPS) to trade-off photorealism and physical-consistency%, while, due to simplicity, not respecting sample diversity. 

%, and 2) compare the two models against a variety of existing metrics to identify the model that best balances photorealism and physical consistency. 
%We will compare the models and metrics by creating a library for qualitative and quantitative assessment of images with the following metric-driven validity checks:


%We will assess existing metrics to compose a novel metric, which balances the photorealism and validity of physically-modeled flood extent in generated imagery.

%\textbf{Photorealism} Image should look photorealistic.  Baseline: Discriminator loss. We use LPIPS (i.e., MSE in AlexNet feature space) (among source and target images)~\cite{Zhang_2018}

%\textbf{Physical consistency} Post-flood image should reconstruct a large part of the pre-flood image. The baseline is Pixel-based reconstruction loss for the target, which will cause issues due to pixel misalignment. We use Intersection over Union (IoU) of a flood segmentation mask from generated and real post-flooding image, which will require a flood segmentation model.

